Enhanced quantum state transfer via feedforward cancellation of optical phase noise

Many experimental platforms for quantum science depend on state control via laser fields. Frequently, however, the control fidelity is limited by optical phase noise. This is exacerbated in stabilized laser systems where high-frequency phase noise is an unavoidable consequence of feedback. Here we implement an optical feedforward technique to suppress laser phase noise in the STIRAP state transfer of ultracold RbCs molecules, across 114 THz, from a weakly bound Feshbach state to the rovibrational ground state. By performing over 100 state transfers on single molecules, we measure a significantly enhanced transfer efficiency of 98.7(1)% limited only by available laser intensity.

==> Abstract.tex <==
% We demonstrate an enhancement in state transfer efficiency in RbCs molecules, by suppressing laser phase noise with an opto-electronic feedforward technique. Laser phase noise from the servo bump of PDH-locked STIRAP lasers are shown to be a limiting factor for STIRAP efficiency for sufficiently high Rabi frequencies. Feed forward suppression effectively suppresses the servo bump by $\sim \SI{20}{dB}$ on both the pump and stokes lasers. An efficiency advantage is demonstrated with the feedforward suppression and yields $\eta=98.7(1)\%$. We present simulations of the STIRAP Hamiltonian for our experimental conditions and make projections for further efficiency gain.  
We demonstrate an enhancement in the efficiency of Stimulated  Raman Adiabatic Passage (STIRAP)  in RbCs molecules, by suppressing laser phase noise with an opto-electronic feedforward technique. By applying the frequency error signal generated by the widely used PDH technique to an electro-optic modulator after suitable optical delay we are able to achieve real-time correction of the laser frequency and reduce phase noise around the molecular coupling frequency by  $\sim \SI{20}{dB}$. Using molecules prepared in an optical tweezer array we are able to demonstrate a one-way state transfer efficiency of $\eta=98.7(1)\%$. We present numerical simulations accounting for the main noise sources in our experiment which suggest avenues for further gain in efficiency. Our measurements demonstrate the effectiveness of the feedforward technique and show promise for high-fidelity quantum simulation and computation with associated ultracold molecules.

==> Hamiltonian.tex <==
\begin{widetext}
\begin{equation}
H_{\text{BD}} = \frac{1}{2}
\begin{pmatrix}
2 \xi_{S} \sin ^{2} \theta + 2 \xi_{P} \cos ^{2} \theta + \delta \cos 2 \theta & \Omega_{rms} & 2 i \dot{\theta} - (\xi_{S} - \xi_{P} + \delta) \sin 2 \theta \\
\Omega_{rms} & -2 \Delta - i \gamma & 0 \\
-2 i \dot{\theta} - (\xi_{S} - \xi_{P} + \delta) \sin 2 \theta & 0 & 2 \xi_{S} \sin ^{2} \theta + 2 \xi_{P} \cos ^{2} \theta - \delta \cos 2 \theta
\end{pmatrix},
\label{eq:HBD}
\end{equation}
\end{widetext}

